Capacity of All Nine Models of Channel Output Feedback for the Two-user Interference Channel

In this paper, we study the impact of different channel output feedback architectures on the capacity of the two-user interference channel. For a two-user interference channel, a feedback link can exist between receivers and transmitters in 9 canonical architectures (see Fig. 2), ranging from only one feedback link to four feedback links. We derive the exact capacity region for the symmetric deterministic interference channel and the constant-gap capacity region for the symmetric Gaussian interference channel for all of the 9 architectures. We show that for a linear deterministic symmetric interference channel, in the weak interference regime, all models of feedback, except the one, which has only one of the receivers feeding back to its own transmitter, have the identical capacity region. When only one of the receivers feeds back to its own transmitter, the capacity region is a strict subset of the capacity region of the rest of the feedback models in the weak interference regime. However, the sum-capacity of all feedback models is identical in the weak interference regime. Moreover, in the strong interference regime all models of feedback with at least one of the receivers feeding back to its own transmitter have the identical sum-capacity. For the Gaussian interference channel, the results of the linear deterministic model follow, where capacity is replaced with approximate capacity.

==> figs/discuss.tex <==
\section{Discussion}
\label{sec:discuss}
In this Section, intuitive explanations are provided for the results
presented in Section \ref{sec:deterministic} and
\ref{sec:gaussian}. The insights are gained from observing the linear
deterministic channel closely. The discussion is based on
understanding the single direct link feedback model at each step and
subsequently extending the insights to other feedback models. We offer
explanations for equivalence the sum-capacity of several feedback
models and the reason for existence of the bound ($2R_1 + R_2$) and
its non existence is some other feedback models. We also offer some
explanation regarding why different regimes of interference experience
different gains from feedback.

The single direct link feedback model is characterized by four
bounds. This is unlike the interference channel without feedback
\cite{bresler2,costa82,etkin} which is characterized by five bounds or
interference channel with conventional feedback
\cite{suh-allerton,suh-2009}, which is characterized by three
bounds. In the single direct link feedback model one of the $R_1 +
2R_2$ or $2R_1 + R_2$ is deactivated based on whether
receiver-transmitter pair $\mathsf{D_1}-\mathsf{T_1}$ or
$\mathsf{D_2}-\mathsf{T_2}$ respectively communicate via a feedback
link.


The single direct link feedback has two advantages. First, the
sum-capacity of the IC with one direct link feedback is larger than
the sum-capacity without feedback. The sum-capacity with one direct
link feedback is same as the sum-capacity of feedback model with all
four links of feedback. In different regimes of interference, this
increase can be attributed to different reasons. We explain the
intuition behind this with examples. Consider, the interference
channel model in Fig. \ref{fig:discuss_1}, where $n = 3, m =1$ (weak
interference). The first three blocks transmission of an achievability
scheme which achieves corner point $(2,3)$ has been depicted. In the
weak interference regime, without the feedback, treating interference
as noise is a good scheme. In the deterministic model, this is
analogous to saying that in the second block either $a_2$ or $b_4$ can
be transmitted but not both, as they interfere with each other. With
feedback, however, the transmitter $\mathsf{T}_1$ transmits $b_4$ in
the $3^\mathrm{rd}$ block to help its receiver $\mathsf{D}_1$ resolve
the interference and obtain $a_2$. At the same time, since $b_4$ is
already decoded at receiver in the $2^\mathrm{nd}$ block, and thus it
is simply be subtracted from the received message at $\mathsf{D}_2$ in
the $3^\mathrm{rd}$ block. Thus transmitting $b_4$ on the top bit of
$\mathsf{T}_1$ potentially allows transmission without interference
and hence adds an additional bit to the sum-rate. In an interference
channel where $m < \frac{n}{2}$, $\mathsf{T}_1$ can retransmit as many
as $m$ $bits$ out of the $n$ bits transmitted by $\mathsf{T}_2$ in the
previous block. The bits being retransmitted can be retransmitted at
the top $m$ bit locations of $\mathsf{T}_2$ so as to help
$\mathsf{D}_1$ resolve interference. Since $\mathsf{D}_2$ will have
decoded all the $m$ $bits$ in the previous block, $\mathsf{T}_2$ can
continue to transmit as many as $m$ additional $bits$ on those bit
locations where the retransmitted bits are being received at
$\mathsf{D}_2$. These $m$ $bits$ are decoded by subtracting out the
retransmitted bits. An increase of $m$ $bits$ in the sum-capacity is
therefore possible.

Now we wish to answer the question of whether adding more feedback
will lead to more improvement in the sum-capacity? The total number of
interfering locations (at $\mathsf{D}_1$ and $\mathsf{D}_2$ combined)
is $2m$. From the achievable scheme, it is noticeable that if a subset
of bits, say $\delta$ in number, are retransmitted by $\mathsf{T}_1$
in each block (in the example in Fig \ref{fig:discuss_1}, $\delta =
1$), it can help resolve as many interference caused at $\delta$ bit locations
previous block. If $\delta$ retransmission happen, then the locations
where potential interference is caused are $2m - \delta$. It is
natural to pick $\delta = 2m - \delta$, thus resolving all the
interference. Even with more than one feedback link this limitations
hold true and thus adding additional feedback link does not improve
the sum-capacity.
\begin{figure}
\centering \subfigure[a]{\label{fig:discuss_1}
\resizebox{3.0in}{!}{\input{discuss_1.pdf_t}}}\hspace{2cm}
\subfigure[b]{\label{fig:discuss_2}
\resizebox{3.0in}{!}{\input{discuss_2.pdf_t}}}
\caption{First three blocks of corner point achieving strategy}
\label{fig:discuss_reg1}
\end{figure}
We also observe that $2R_1 + R_2$ is an active bound in this
regime. Notice that, if the transmitter $\mathsf{T}_1$ tries to
transmit one of its own message bits, say $a_5$ (as depicted in
Fig. \ref{fig:discuss_2}), instead of $b_4$, it causes interference at
$\mathsf{D}_2$, at the same time \emph{not} helping remove the
interference from $a_2 \oplus b_4$. Thus transmission of one additional
$bit$ at $\mathsf{T}_1$ causes a total loss of two $bits$. In fact in
order to avoid any interference in the $2^\mathrm{nd}$ block,
$\mathsf{T}_2$ should not transmit $b_4$ and $b_6$. An increase of one
$bit$ in the rate $R_1$ is therefore equivalent to loss of 2 $bits$ in
$R_2$, thus pointing at the existence of a possible $2R_1 + R_2$
bound.

Once again, note that the burden of retransmissions (such that one of
the receivers, $\mathsf{D}_1$ benefits without $\mathsf{D}_2$ loosing
anything) is entirely on the the transmitter $\mathsf{T}_1$. More
generally, the burden is on the transmitter receiving feedback. As
long as only $\mathsf{T}_1$ receives feedback, the $2R_1 + R_2$ bound
does not seem to relax. However, when both $\mathsf{T}_1$ and
$\mathsf{T}_2$ receive feedback (from either/both receivers), part of
the retransmission can be handled by $\mathsf{T}_1$ (say $\gamma$) and
the rest (i.e. $m - \gamma$) by $\mathsf{T}_2$. Thus, other points on
the sum-capacity achieving line are also feasible, and therefore $2R_1
+R_2$ bound is also deactivated (as observed in the case of single
receiver broadcast, conventional feedback or four link feedback model).

\begin{figure}
\centering \subfigure[Sum-capacity achieving scheme in the \emph{no}
feedback model,{$n = 5, m = 3$}]{\label{fig:discuss_3}
\resizebox{1.5in}{!}{\input{discuss_6.pdf_t}}}\hspace{2cm}
\subfigure[First three stages of sum-capacity achieving strategy in the
single direct link feedback model]{\label{fig:discuss_4}
\resizebox{2.9in}{!}{\input{discuss_7.pdf_t}}}
\caption{Sum-capacity achieving schemes with and without feedback}
\label{fig:discuss_reg2}
\end{figure}
Consider another example depicted in the Fig.\ref{fig:discuss_reg2}
($n = 5, m= 3$). In this regime, good schemes in interference channel
without feedback employ common messages being transmitted by both the
transmitters. For instance, in the example in the
Figure \ref{fig:discuss_3}, $a_1$ and $b_1$ are common messages. It is
clear that, in order to improve the sum-rate, retransmission, of a
part of the message transmitted by $\mathsf{T}_2$ in the
$i^\mathrm{th}$ block, in the $(i+1)^\mathrm{th}$ block by
$\mathsf{T}_1$ is important. It is also clear that the retransmitted
$bit$ has already been decoded at $\mathsf{D}_2$ in $i^\mathrm{th}$
block, while it should be decodable at $\mathrm{D}_1$ in the
$(i+1)^\mathrm{th}$ block. This ensures resolving interference at
$\mathsf{D}_1$ without causing new interference at $\mathsf{D}_2$. In
order to ensure decoding of an additional bit $\mathsf{D}_2$, the it
should be transmitted from $\mathsf{T}_2$ only from those bit
locations where the received bit at $\mathsf{D}_2$ in
Fig. \ref{fig:discuss_3} was 0. Similarly, the retransmission from
$\mathsf{T}_1$ should happen from bit locations where 0 was being
received $\mathsf{D}_1$ in Figure \ref{fig:discuss_3}. Thus the
maximum increase in the sum-rate possible is bottle-necked by the
minimum of such locations, which turns out to 1 in the example in
Figure \ref{fig:discuss_3}. In general, for arbitrary $m,n$ where $m >
\frac{n}{2}$, this number is $(2n - 3m)^+$. An example of this
achievability scheme is shown in Figure \ref{fig:discuss_4} clearly
showing a gain of $(2n -3m)^+ = 1$ bit in sum-rate (in every stage 3
and 4 new bits are decoded at $\mathsf{D}_1$ and $\mathsf{D}_2$
respectively). Note that, for $m \geq \frac{2n}{3}$, $(2n - 3m)^+ =
0$, thus explaining no gain in that regime. Once again, note that this
bottle neck is independent of whether there is a single direct link
feedback or more. Thus, the sum-capacity of single direct link
feedback is same as that of single receiver broadcast feedback or four
link feedback model. The $2R_1 + R_2$ bound however, as discussed
earlier, still exists for the single direct link feedback model, while
can be easily deactivated by sharing the burden of retransmission
between the two transmitters.

In the regime where interference is very strong, gain in the
sum-capacity is natural because of the possible relay route (for the
message at $\mathsf{T}_2$) from $\mathsf{T}_2 \to \mathsf{D}_1 \to
\mathsf{T}_1 \to \mathsf{D}_2$. Since the relay path can support
higher rates than the direct link ($m > n$, or analogously
$\mathsf{INR > SNR}$), therefore the sum-capacity with single direct
link feedback is larger than that without feedback. Note that, since
the feedback link is of infinite capacity, the bottleneck of the
increase in the rate of transmission from $\mathsf{T}_2 \to
\mathsf{D}_2$ is the minimum rate that can be supported by the
interfering links (cross links). Since each of the cross links can
support $m$ $bits$, the relaying mechanism can allow as many as $m$
$bits$ being transmitted between $\mathsf{T}_2$ and $\mathsf{D}_2$
(note that $m > n$). With an additional feedback link, say between the
second receiver-transmitter receiver pair, another relay path
$\mathsf{T}_1 \to \mathsf{D}_2 \to \mathsf{T}_2 \to \mathsf{D}_1$ is
possible. The bottleneck of increase in the total rate of transmission
remains the same as case when there was only one direct link
feedback. Moreover, both the relay paths have parts $\mathsf{T}_1 \to
\mathsf{D}_2$, $\mathsf{T}_2 \to \mathsf{D}_1$ in common. The total
number of bits that can be pushed through them does not increase with
more feedback links and hence the increase in sum-capacity is the same
as when there is only one direct link feedback. However, adding an
additional direct feedback link (between $\mathsf{T}_2$ and
$\mathsf{D}_2$) implies an increase in the rate of transmission at
both the transmitters, it implies a larger capacity region
too. However, the cross link feedback does not any additional relay
path, therefore the capacity region of deterministic interference
channel with or without the cross link feedback is the same. Thus, in
the strong interference regime single direct link feedback and single
receiver broadcast feedback models have the same capacity region.




==> references.tex <==
\begin{thebibliography}{10}
%% \bibitem{shannon56} C. E. Shannon, ``The zero error capacity of a
%% noisy channel,'' {\em IRE Trans. Inf. Th.,} Sept.
%% 1956.


%% \bibitem{ozarowmac} L. Ozarow, ``The capacity of the white Gaussian
%%   multiple access channel with feedback,'' {\em IEEE Trans. Inf. Th.,}
%%   vol 30, no. 4, Jul. 1984.


%% \bibitem{ozarowbc} L. Ozarow, S. Leung-Yan-Cheong, ``An achievable
%% region and outer bound for the Gaussian broadcast channel with
%% feedback,'' {\em IEEE Trans. Inf. Th.}, vol.30, no.4, pp. 667-671, Jul.
%% 1984.

%% \bibitem{carleial} A. Carleial, ``Multiple-access channels with
%% different generalized feedback signals,'' {\em IEEE Trans. Inf. Th.},
%% vol.28, no.6, Nov. 1982.


%% \bibitem{bhaskaran} S. R. Bhaskaran, ``Broadcasting with feedback,''
%%   in Proc. {\em IEEE International Symposium Information Theory}, Jun.
%%   2007, Nice, France.


\bibitem{costa85} M. H. M. Costa, ``On the Gaussian interference
  channel,” IEEE Trans.~Inf.~Th., vol. IT-31, no. 5, Sep. 1985.

\bibitem{sato78} H. Sato, ``On degraded Gaussian two-user channels,”
IEEE Trans. Inf.  Theory, vol. IT-24, no. 5, Sep. 1978.

\bibitem{sason} I. Sason, ``On Achievable Rate Regions for the Gaussian
Interference Channel,'' {\em IEEE Trans. Inf. Theory,} vol. 50,
no. 6, June 2004.

\bibitem{etkin} R. Etkin, D. Tse, and H. Wang, ``Gaussian interference
  channel capacity to within one bit,'' {\em IEEE Trans. Inf. Th.},
  vol. 54, no. 12, Dec. 2008.

%% \bibitem{araja} A. Raja, V. M. Prabhakaran, and P. Viswanath, ``The two
%% user Gaussian compound interference channel,'' {\em IEEE
%%   Trans. Inf. Th.} vol. 55(11), November 2009


\bibitem{sato} H. Sato, ``The capacity of the Gaussian interference
channel under strong interference,'' {\em IEEE Trans. Inf. Theory}
vol. IT-27, no.6, Nov.~1981.

\bibitem{car} A.B. Carleial, ``A case where interference does not
reduce capacity,'' {\em IEEE Trans. Inf. Theory}, vol. IT-21, no.5,
Sept. 1975.

%% \bibitem{jafar} V. Cadambe, S.A. Jafar, and S. Shamai, ``Interference
%% alignment on the deterministic channel and application to fully
%% connected AWGN interference networks,'' { \em IEEE Information Theory
%% Workshop (ITW), 2008} pages 41- 45, 2008.

\bibitem{costa82} M. H. M. Costa and A. El Gamal, ``The capacity
region of a class of deterministic interference channels,'' { \em IEEE
Trans. Inform. Theory}, vol. 28, no. 2, pp. 343 -346, Mar. 1982.

\bibitem{bresler2} G. Bresler and D. Tse, ``The two-user Gaussian
interference channel: A deterministic view,'' {\em
Euro. Trans. Telecomm.,} vol. 19(4), pp. 333-354, June 2008.

\bibitem{kramer02} G. Kramer, ``Feedback strategies for white Gaussian
interference networks,'' {\em IEEE Trans. Inf. Th.},
vol. 48, pp. 1423-1438, June 2002.

\bibitem{kramer04} G. Kramer, ``Correction to ``Feedback strategies
for white Gaussian interference networks'', and a capacity theorem for
Gaussian interference channels with feedback,'' {\em IEEE Trans.
Inf. Th.}, vol. 50, June 2004.

\bibitem{gast06} M. Gastpar and G. Kramer, ``On noisy feedback for
interference channels,'' {\em in Proc. Asilomar Conference on Signals,
Systems, and Computers}, Oct. 2006.

\bibitem{jiang07} J. Jiang, Y. Xin, and H. K. Garg, ``Discrete
memoryless interference channels with feedback,'' {\em in Proc. CISS
41st Annual Conference}, pp. 581-584, Mar. 2007.


\bibitem{tuninetti} D. Tuninetti, ``The Interference Channel with
  Generalized Feedback (IFC-GF),'' {\em ITA Workshop}, UCSD, 2006.

\bibitem{tunita} D. Tuninetti, ``An outer bound region for Interference
  Channels with Generalized Feedback,'' {\em ITA Workshop}, UCSD 2010


\bibitem{prabhakaran-sc} V. Prabhakaran and
  P. Viswanath, ``Interference Channel with Source Cooperation,'' IEEE
  Transactions on Information Theory, vol. 57, no. 1, pp. 156-186,
  January 2011.

\bibitem{tunout} S. Yang and D. Tuninetti, ``A new sum-rate outer bound for Gaussian
  Interference Channels with Generalized Feedback,'' {\em IEEE
    International Symposium on Information Theory 2009}, Seoul, South
  Korea, June 2009.

\bibitem{tuninetti-sc} S. Yang and D. Tuninetti, ``Interference Channel With Generalized
  Feedback (a.k.a. With Source Cooperation): Part I: Achievable
  Region,''{\em IEEE Trans. Inf. Th.}, vol. 57, 2011, pages 2686-2710.

\bibitem{madsen}
Anders Høst-Madsen, ``Capacity Bounds for Cooperative Diversity,'' {\em
IEEE Trans. Inf. Th.}, Vol. 52, No. 4, April 2006.

\bibitem{suh2009}
C. Suh and D.N.C. Tse, ``Feedback Capacity of the Gaussian
Interference Channel to Within 2 Bits,'' \emph{IEEE Trans. Inf. Th.},
vol.57, no.5, pp.2667-2685, May 2011

\bibitem{suh-allerton}
C. Suh and D.N.C. Tse, ``The feedback capacity
region of El-Gamal deterministic interference channel,'' {\em in
Proceedings of 47th Annual Allerton Conference on Communication,
Control and Computing}, September 2009.

\bibitem{avestimehr} A. S. Avestimehr, S N. Diggavi and D N
C. Tse, ``Wireless network information flow: A deterministic
approach,'' {\em IEEE Trans. Inf. Theory}, vol. 57,  pp.1872 - 1905 , 2011.

\bibitem{dirtypaper} M. H. M. Costa, ``Writing on dirty paper,'' {\em
    IEEE Trans. Info. Th.}, pp. 439 - 441, May
  1983. Trans.

\bibitem{coverbook} T. M. Cover and J. A. Thomas, {\em Elements of
Information Theory}. Wiley Series in Telecommunications and Signal
Processing, $2^\mathrm{nd}$ edition, 2006.

\bibitem{relay} T. M. Cover and A.E. Gamal, ``Capacity theorems for
the relay channel,'' {\em IEEE Trans. Inf. Th.},
vol. 25, no. 5, pp. 572-584, Sep 1979.

\bibitem{schur} F. Zhang, {\em The Schur Complement and its
Applications}, Springer, vol.4, 2005.

\bibitem{asahai1} A. Sahai, V. Aggarwal, M. Yuksel, A. Sabharwal, ``On
channel output feedback in deterministic interference channel,'' {\em
in Proc. of Information Theory Workshop,}, Taormina, Italy, October
2009.

\bibitem{asahai2} A. Sahai, V. Aggarwal, M. Yuksel, A. Sabharwal,
``Sum capacity of general deteministic interference channel with
channel output feeback,'' {\em to appear in Proc. of International
Symposium of Information Theory}, Austin, USA, June 2010.

\bibitem{alireza} A. Vahid, C. Suh, A. S. Avestimehr, ``Interference
  Channels with Rate-Limited Feedback,'' {\em to appear IEEE
    Trans. Inf. Th.}, March 2011.

\bibitem{han} T. S. Han and K. Kobayashi, ``A new achievable rate
region for the interference channel,'' {\em IEEE Trans. Inf. Th.},
vol. 27, no. 1, pp. 49-60, Jan. 1981.


\end{thebibliography}

